Is Reinforcement Learning (Not) for Natural Language Processing: Benchmarks, Baselines, and Building Blocks for Natural Language Policy Optimization

We tackle the problem of aligning pre-trained large language models (LMs) with human preferences. If we view text generation as a sequential decision-making problem, reinforcement learning (RL) appears to be a natural conceptual framework. However, using RL for LM-based generation faces empirical challenges, including training instability due to the combinatorial action space, as well as a lack of open-source libraries and benchmarks customized for LM alignment. Thus, a question rises in the research community: is RL a practical paradigm for NLP? To help answer this, we first introduce an open-source modular library, RL4LMs (Reinforcement Learning for Language Models), for optimizing language generators with RL. The library consists of on-policy RL algorithms that can be used to train any encoder or encoder-decoder LM in the HuggingFace library (Wolf et al. 2020) with an arbitrary reward function. Next, we present the GRUE (General Reinforced-language Understanding Evaluation) benchmark, a set of 6 language generation tasks which are supervised not by target strings, but by reward functions which capture automated measures of human preference. GRUE is the first leaderboard-style evaluation of RL algorithms for NLP tasks. Finally, we introduce an easy-to-use, performant RL algorithm, NLPO (Natural Language Policy Optimization) that learns to effectively reduce the combinatorial action space in language generation. We show 1) that RL techniques are generally better than supervised methods at aligning LMs to human preferences; and 2) that NLPO exhibits greater stability and performance than previous policy gradient methods (e.g., PPO (Schulman et al. 2017)), based on both automatic and human evaluations.

==> tex/main/grue.tex <==
We introduce \longname (\shortname), a benchmark that contains a collection of resources pertaining to issues and potentially solutions for training, tuning, and evaluating RL for text-generation.

\subsection{Potential Pitfalls of Reinforcement Learning  \kb{Something more catchy?}}
Though reformulating NLP tasks seems enticing, there has been some problems and concerns mention in the literature \kb{A better catchy phrase}. 
\textcolor{blue}{(1)} In, past issues, regarding optimizing a reward for language (especially for a metric) does not guarantee an increase in the quality of the output \citep{paulus2017deep} (i.e. reward hacking \citep{}). 
\textcolor{blue}{(5)} In addition, issues around solving a sparse reward problem for text-generation \citep{Choshen2020On}. (6)
\textcolor{blue}{(2)} \kb{[Raj check this $\rightarrow$] Also, concerns around RL is only likely to improve over pre-trained models when the pre-trained is already performing well \citep{Choshen2020On}; including using the KL penalty and staying extremely close to the pre-trained model\citep{korbak2022controlling} }.
\textcolor{blue}{(3)} RL methods have high variance and instability in the objective function \citep{wu2018study,li-etal-2017-adversarial, wu2016google}. 
\textcolor{blue}{(4)} The action space in RL for text-generation is high dimensional and combinatorial (size of the vocabulary) \citep{Choshen2020On}. 
\textcolor{blue}{(5)} \kb{[Raj check this $\rightarrow$] RL methods suffer from loss of capabilities of the original model} \citep{korbak2022controlling}. 
\textcolor{blue}{(6)} \kb{[Raj check this $\rightarrow$] Sum of actions for rewards not equal to the overall metrics, forcing a discount factor $\discount \approx 1$, in most RL for text-generation experiments \citep{}} 
\textcolor{blue}{(7)} \kb{[Raj check this $\rightarrow$] Extremely high initial state distribution $\initialstate$ due to prompts needed for encoder-decoders to reduce instability with PPO. } \citep{}.
Although some of these issues has been addressed only in the context of Neural Machine Translation (NMT) \citet{samuel2021revisiting}, this evaluation focuses on a broader set of text-generation task.





\subsection{Guidelines on When to Use RL for Text-Generation}
What is RL good for in the context of language? Metric optimization (be careful), sequential tasks, intermediate rewards - incorporating feedback (interactivity), goal driven generation, already have a good init policy via pretraining


part of the fix is the KL penalty, but let's think about MDP sample complexity, that depends on gamma too




\subsection{Tasks and Metrics}

\begin{table*}[t!]
  \small
  \begin{center}
  \begin{tabular}{@{}m{8.2em}m{11.2em}m{5em}rm{5em}rm{3em}rm{3em}@{}}
  \toprule
       \textbf{Dataset}
     & \textbf{Task}
     & \centering\arraybackslash \textbf{Language(s)}
     & \textbf{Size}
     & \centering\arraybackslash\textbf{Input Type} 
     & \centering\arraybackslash\textbf{\textcolor{red}{Done}}\\
  \toprule
      \makecell[bl]{\small{CommonGEN}\\ \small{\citep{lin2019commongen}}}
      & \small{Generative Commonsense}
      & \centering\arraybackslash\small{en} 
      & \centering\arraybackslash\small{67k} 
      & \centering\arraybackslash\small{Concept Set} 
      & .
      & Y
      \\ 
  \midrule
      \makecell[bl]{\small{CNN Daily Mail}}
      & \small{Summarization}
      & \centering\arraybackslash\small{en} 
      &  \centering\arraybackslash\small{287k}
      &  \centering\arraybackslash\small{News Article} 
      & .
      & Y
      \\
  \midrule
      \makecell[bl]{\small{IMDB}\\ } 
      & \small{Text Continuation}
      &  \centering\arraybackslash\small{en}
      &  \centering\arraybackslash\small{25k}
      & \centering\arraybackslash\small{Partial Movie Review} 
      & . %
      & Y
      \\
  \midrule
      \makecell[bl]{\small{ToTTo}\\ \small{\citep{parikh2020totto}}} 
      & \small{Data to Text}
      & \centering\arraybackslash\small{en} 
      & \centering\arraybackslash\small{136k}  
      & \centering\arraybackslash\small{Highlighted Table}
      & .
      & Y
      \\
  \midrule
      \makecell[bl]{\small{WMT-19}} 
      & \small{Machine Translation}
      & \centering\arraybackslash\small{en, ru, de, fr} 
      & \centering\arraybackslash\small{-}  
      & \centering\arraybackslash\small{Text}
      & .
      & Y
      \\
  \midrule
      \makecell[bl]{\small{NarrativeQA}}
      & \small{Question Answering}
      & \centering\arraybackslash\small{en} 
      & \centering\arraybackslash\small{-}  
      & \centering\arraybackslash\small{Question Context}
      & .
      & Y
      \\
  \bottomrule
  \end{tabular}
  \end{center}
  \caption{}
  \label{tab:overview}
\end{table*}




\subsection{On-Policy Algorithms for Generation}

how do we actually get these to work, what's the key idea - restrict optimization to trust region of "natural language"

well, that's slow - so we use the KL penalty which 

generic actor critic for generation psuedocode

the calculate returns line varies based on PPO vs A2C. TRPO straight up does second order

